Sequential Recommendation with Self-Attentive Multi-Adversarial Network

Recently, deep learning has made significant progress in the task of sequential recommendation. Existing neural sequential recommenders typically adopt a generative way trained with Maximum Likelihood Estimation (MLE). When context information (called factor) is involved, it is difficult to analyze when and how each individual factor would affect the final recommendation performance. For this purpose, we take a new perspective and introduce adversarial learning to sequential recommendation. In this paper, we present a Multi-Factor Generative Adversarial Network (MFGAN) for explicitly modeling the effect of context information on sequential recommendation. Specifically, our proposed MFGAN has two kinds of modules: a Transformer-based generator taking user behavior sequences as input to recommend the possible next items, and multiple factor-specific discriminators to evaluate the generated sub-sequence from the perspectives of different factors. To learn the parameters, we adopt the classic policy gradient method, and utilize the reward signal of discriminators for guiding the learning of the generator. Our framework is flexible to incorporate multiple kinds of factor information, and is able to trace how each factor contributes to the recommendation decision over time. Extensive experiments conducted on three real-world datasets demonstrate the superiority of our proposed model over the state-of-the-art methods, in terms of effectiveness and interpretability.

==> Sequential Recommendation with Self-Attentive Multi-Adversarial Network/subfile2/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Recommender systems aim to accurately characterize user interests and provide personalized recommendations in a variety of real-world applications. They serve as an important information filtering technique  to alleviate the information overload problem and enhance user experiences. 
In most applications, users' interests are dynamic and evolving over time.
It is essential to  capture the dynamics of sequential user behaviors for making appropriate recommendations.
%, influenced by their historical behaviors. 
%For example, a user may purchase cell phone accessories (\eg mobile phone cases) soon after buying an iPhone. %, while she/he will not buy any cases under normal circumstances.


In the literature, various methods \cite{RendleFS10, GRU4Rec, kang2018self} have been proposed for sequential recommender systems. 
Early methods usually utilize the Markov assumption that the current behavior is tightly related to the previous ones~\cite{RendleFS10}.
Recently, sequential neural networks such as recurrent neural network~\cite{GRU} and Transformer~\cite{transformer} have been applied to recommendation tasks as these networks can  characterize sequential user-item interactions and  learn effective representations of user behaviors~\cite{GRU4Rec, kang2018self}. Besides, several studies have proposed to incorporate context information to enhance the  performance of neural sequential recommenders~\cite{GRU-f, li2019review, HuangWSDM19}. The advantages of these sequential neural networks have been experimentally confirmed as they have achieved significant performance improvements.



Typically,  existing neural sequential  recommenders~\cite{kang2018self, GRU4Rec} adopt a generative way to predict future items and learn the parameters using Maximum Likelihood Estimation~(MLE).
%When context information is utilized, it has to be integrated with the original recommendation component~\cite{GRU-f}. 
However, it has been found that MLE-based training is easy to suffer from issues such as data sparsity or exposure bias~\cite{Ranzato2015Sequence,Yu2017SeqGAN} in sequence prediction.
Especially, in such an approach,  when context information  (called as \emph{factor} in this paper) is incorporated, it has to be integrated with the original sequential prediction component~\cite{GRU-f,HuangWSDM19, li2019review}. %Various factors (\eg price and brand of a product in the e-commerce scenario) are either mixed in the sequential context representations, or coupled with the black-box recommendation module.  
The consequence is that  various factors (\eg price and brand of a product in the e-commerce scenario) are either mixed in the sequential context representations, or coupled with the black-box recommendation module.  Therefore, we cannot accurately figure out when and how each individual factor would affect the final recommendation performance. 
These disadvantages weaken or even impede their applications in a wide range of  decision making scenarios. 
It is important to explicitly and effectively characterize the effect of various factors in sequential recommender systems. %It is the key to improve the performance and enhance the interpretability of sequential recommenders. 


\ignore{More importantly, when context information  (called as \emph{factor} in this paper) is utilized, it has to be integrated with the original sequential prediction component~\cite{GRU-f,HuangWSDM19, li2019review}.
In such  a way,  various factors (\eg price and brand of a product in the e-commerce scenario) are either mixed in the sequential context representations, or coupled with the black-box recommendation module.  
Therefore, we cannot accurately figure out when and how each individual factor would affect the final recommendation performance. 
These disadvantages weaken or even impede their applications in a wide range of business decision making. 
It is essential to be able to explicitly and effectively characterize the effect of various factors on users' sequential behaviors. 
}%It is the key to improve the performance and enhance the interpretability of sequential recommenders. 


\ignore{
We argue that it is not the most suitable to seek interpretable recommendation with available factor information.    
However, these sequential neural networks also pose great challenges in understanding the sequential characteristics of user behaviors due to the black-box nature of deep neural networks.
Even with supplementary context information (called as \emph{factor} in this paper), it is still difficult to understand the reasons behind the recommendation outputs.
%Typically,  existing neural sequential  recommenders~\cite{} adopt a generative way to make the item recommendation and learn the parameters using Maximum Likelihood Estimation~(MLE).
%It is difficult to  incorporate useful factor information into such an architecture in an interpretable  way.    
In existing context-aware sequential recommendation algorithms~\cite{GRU-f, HuangWSDM19, li2019review, chen2016learning},
various factors, such as price and brand of a product in the e-commerce scenario, or genres and actors of a movie in the movie scenario, are either mixed in the sequential context representations, or coupled with the black-box recommendation module.  
 %and then are further modeled by neural networks in a black-box manner.
}

%Therefore, %We cannot accurately understand the reasons behind the recommendation outputs, or study how some specific factor affects the 
%valuable patterns within behavior sequences are also hard to identify.


%that lead to various behavior sequences and further improve the performance of recommender systems and enhance the user experience.
 



In the light of this challenge, we propose to use an adversarial training approach to developing sequential recommender systems. 
Indeed, the potential advantage of Generative Adversarial Network~(GAN) has been shown in  collaborative filtering methods~\cite{CFGAN,IRGAN}. Different from prior studies, our novelty is to  decouple  \emph{factor utilization} from the \emph{sequence prediction} component via adversarial training.
%we take a new perspective   to incorporate useful context information in sequential recommendation. 
Following the GAN framework~\cite{GAN-2014-NIPS}, we set two different components, namely generator and discriminator. 
In our framework, 
the generator predicts the future items for recommendation relying  on user-item interaction data alone, while the discriminator  judges the rationality of the generated recommendation sequence based on available  information of various factors.
Such an approach allows more flexibility in utilizing external context information in sequential recommendation, which is able to improve the recommendation interpretability. 
%The major novelty of our work is to decouple  \emph{factor utilization} from the \emph{sequence prediction} component, which is able to improve the recommendation interpretability. 

% The potential advantage of GAN has been shown in  collaborative filtering methods~\cite{CFGAN,IRGAN}, while we take a new perspective to improve the sequential recommendation. 

%Besides model learning, the  adversarial training approach allows more flexibility in utilizing external context information for the recommendation interpretability.  Via adversarial training, the major motivation of our work is to decouple  \emph{factor utilization} from the \emph{sequence prediction} component. 


\ignore{we propose  a novel \emph{Multi-Factor Generative Adversarial Network (MFGAN)}. 
Our core idea is to decouple  \emph{factor utilization} from the \emph{sequence prediction} component. 
We
set supplementary evaluation components to incorporate the factor information, and further  help improve the original generator component.  We set multiple evaluation components and associate each one with a specific kind of factor information. 
In this way, factor information has not  been directly involved in the generative process, and only serves to provide useful signal to guide the learning of the original generation component.
%This method decouples   \emph{factor utilization} from the \emph{recommendation} component.  
%In this way, we can decouple  \emph{recommendation} and \emph{factor modeling}.   
%set two kinds of components, namely the prediction component and the evaluation component. The prediction component directly generates users' future behaviors based on sequential characteristics; while the evaluation component is mainly used to evaluate the quality of the generated recommendation sequence. 
%In order to accurately understand underlying user preference, we construct multiple evaluation components according to different factors. In this way, we can flexibly incorporate multiples kinds of factors and monitor how a user's behavior evolves \emph{w.r.t.} some specific factor.  
The above idea can be naturally modeled by the Generative Adversarial Network (GAN) framework. 
GAN~\cite{GAN-2014-NIPS} is originally proposed to mimic the generation process of given data samples.
The discriminator in GAN is responsible for providing guidance to the generator by classifying whether a sample is generated or not, while the generator acts as an attacker who constantly provides harder and harder negative samples to the discriminator.
By playing such min-max game, both discriminator and generator become stronger and learn from the given data.  
}

To this end, in this paper, we present  a novel \emph{Multi-Factor Generative Adversarial Network (MFGAN)}. 
Specifically, our proposed MFGAN has two essential kinds of modules: (1) a Transformer-based generator taking user behavior sequences as input to recommend the possible next items, and (2) multiple factor-specific discriminators to evaluate the generated recommendations from the perspectives of different factors.
%For each discriminator, we assign a specific discriminative task with a factor such as item category and price.
Unlike the generator,  the discriminator adopts a bi-directional Transformer-based architecture, and it can refer to the information of subsequent positions for sequence evaluation.
In this way, the discriminator is expected to make more reliable judgement by considering the overall sequential characteristics  \emph{w.r.t.} different factors.
%In this way, the discriminator is more capable of modeling the overall sequential characteristics \emph{w.r.t.} different factors, and derives more reliable evaluation on the generated recommendation sequence. 
Due to the discrete nature of item generation, 
the training of the proposed MFGAN method is realized in a reinforcement learning way by policy gradient. 
The key point is that we utilize the discriminator modules to provide the reward signal for guiding the learning of the generator.

Under our framework, various factors are decoupled from the generator, and they are utilized by the discriminators to derive supervision signals to improve  the generator. 
%With such a design of MFGAN, the information introduced by discriminators provides a seamless way to supervise the generation process for predicting next items, and the signals of classifying generated sub-sequences from multiple discriminators could also serve as the decoupled indicators that which factors determine the current transition behavior.
%We further analyze the effectiveness and the stability of the multi-adversarial architecture in our task, and using multiple discriminators is indeed useful to stabilize the learning process of our approach.
%We discuss four cases to derive the reward from multiple discriminators, and adopt one simple yet more stable way to set the expected reward of a subsequence.  
%\yaliang{to-do: incorporate more details to make this paragraph a bit difficult.}
To validate the effectiveness of the proposed MFGAN, we conduct extensive experiments on three real-world datasets from  different domains. Experimental results show that the proposed MFGAN is able to achieve better performance compared to several competitive methods. 
We further show  the multi-adversarial architecture  is indeed useful to stabilize the learning process of our approach.
Finally, qualitative analysis demonstrates that the proposed MFGAN can explicitly characterize the effect of various factors over time for sequential recommendation, making the recommendation results highly interpretable. 


\eat{
Our main contributions are summarized as follows:
\begin{itemize}[leftmargin=0.1cm,labelsep=.5em, noitemsep]
    \item To the best of our knowledge, we are the first to introduce adversarial training into the sequential recommendation task, unifying the unidirectional generative process and bidirectional discrimination for the recommendation.
    \item We propose a multi-discriminator structure that can decouple different factors and improve the performance of sequential recommendation. We  analyze the effectiveness and the stability of the multi-adversarial architecture in our task.
 %   \item \yaliang{Theoretical analysis states that the structure of multi-discriminator can guarantee the effectiveness and stability of the optimization for generator.}
    \item Extensive experiments conducted on three real-world datasets demonstrate the benefits of the proposed MFGAN over state-of-the-art methods.
\end{itemize}
}


Our main contributions are summarized as follows:

$\bullet$ To the best of our knowledge, we are the first to introduce adversarial training into the sequential recommendation task, and design the unidirectional generator for prediction and bidirectional discriminator for evaluation.

$\bullet$ We propose a multi-discriminator structure that can decouple different factors and improve the performance of sequential recommendation. We  analyze the effectiveness and the stability of the multi-adversarial architecture in our task.
 %   \item \yaliang{Theoretical analysis states that the structure of multi-discriminator can guarantee the effectiveness and stability of the optimization for generator.}

$\bullet$ Extensive experiments conducted on three real-world datasets demonstrate the benefits of the proposed MFGAN over state-of-the-art methods, in terms of both effectiveness and interpretability.


%The rest of this paper is organized as follows. We first formulate the sequential recommendation problem in section~\ref{sec:definition}. After giving an overview of the proposed MFGAN framework, we present the details of model design and  analysis of MFGAN in section~\ref{sec:method}. The experimental results are summarized in section~\ref{sec:exp}, and we conclude the paper in section~\ref{sec:conclusions}.


==> Sequential Recommendation with Self-Attentive Multi-Adversarial Network/subfile2/2_definition.tex <==
\section{Problem Definition}
\label{sec:definition}

In this section, we first formulate the studied problem of sequential recommendation before diving into the details of the proposed method.
Let $\mathcal{U}$ and $\mathcal{I}$ denote a set of users and items, respectively, where $|\mathcal{U}|$ and $|\mathcal{I}|$ are the numbers of users or items.
%The interaction between a user $u \in \mathcal{U}$ and an item $i \in \mathcal{I}$ can be represented by a binary value $0$ or $1$ where $1$ represents the corresponding user and item have an interaction.
Typically, a user $u$ has a chronologically-ordered interaction sequence of items: $\{i_1, i_2, \dots, i_t, \dots, i_{n}\}$, where $n$ is the total number of interactions and $i_t$ is the $t$-th item that user $u$ has interacted with. 
For convenience, we use $i_{j:k}$ to denote the subsequence of the entire sequence, \ie  $i_{j:k}=\{i_j,  \dots, i_k\}$, where $1 \le j < k \le n $.
 Besides, we assume that each item $i$ is associated with $m$ kinds of contextual information, corresponding 
to $m$ factors, \eg artist, album and popularity in music recommender system. 
 
\ignore{
The historical behaviors of each user is denoted by $S_u=\{i_1, i_2, \dots, i_t, \dots, i_{n}\}$ where $i_t \in \mathcal{I}, t \in [1,|u|]$ and $|u|$ is the total number of the user behaviors until the timestamp $t$.
Item $i$ also has a set of features such as product category, movie genre, and music popularity. These features are the factors we discussed above. 
All these features ($i.e.$, factors) are only available for the discriminators in the proposed method as we want to decouple mixed factors through the designed multi-adversarial architecture. More details will be discussed in the next section.
}

Based on the above notations, we now define the task of sequential recommendation.
Formally, given the historical behaviors of a user (\ie $\{i_1, i_2, \dots, i_t, \dots, i_{n}\}$) and the context information of items, our task aims to predict the next item that she/he is likely to interact with at the $(n+1)$-th step.%. \yaliang{define our task upon the sequential recommendation: decoupling multiple factors.}



%In particular, for the information of the knowledge graph, we use the compressed representation from the \textsc{TransE} model~\cite{transe-NIPS-2013}.

==> Sequential Recommendation with Self-Attentive Multi-Adversarial Network/subfile2/3_method.tex <==
\section{Methodology}
\label{sec:method}

In this section, we first give an overview of the proposed \emph{Multi-Factor Generative Adversarial Network}~(MFGAN) framework, and then introduce the design of the generator and discriminators.
The details of the training process are also discussed in this section.

\eat{
\subsection{The MFGAN Framework}
Existing sequential recommendation models are generally generative models~\cite{kang2018self, GRU4Rec}.
During the recommendation process, the sequence of behavior represented by item identifier includes information on different factors, which is difficult to use through the generation process.
In addition, in the generative model, only the items at the previous timestamps can be "seen" at each timestamp, the usage of factor information is also very limited. 

To counter these challenges, we propose an adversarial framework named MFGAN, which has two essential components undertaking different responsibilities for sequential recommendation.
As shown in Figure~\ref{fig-model}, the upper component is the prediction component ($i.e.$ generator $G$) which is a transformer based recommendation model and continuously generate the next items based on the current historical sequence.
The lower component is the evaluation component that is a set of discriminators $\{D_1, D_2, \dots, D_m\}$ to judge the rationality of generated sequence by using the bidirectional information from multiple perspectives.
The two components force each other to improve in a mutual reinforcement way during the training process.
The model design of the discriminator is also based on transformer structure, followed by multiple fully connected layers.
Each discriminator is responsible for a given factor information.

For example, in e-commerce recommender system, we may have the discriminators separately designed for category information, popularity statistic, and item identifier to rate the rationality of transitions by themselves.
The outputs of the discriminators are also returned to the generator side to supervise the learning of the model update in the next round.
Due to the flexibility of two components, it is much easier to add multiple factor information to the discriminators in our framework while it does not affect the generation on the generator side. 
At the same time, the discriminator side can decouple different factor information to interpret transition pattern of user behaviors.
Finally, we use the generator for sequential recommendation tasks.
In the following sections, we will introduce the details of the model design for generator and discriminators.
}


\begin{figure*}[ht]
	\centering 
	\includegraphics[width=0.76\textwidth]{fig/model.pdf}
	\caption{The overview of the proposed MFGAN model consisting of a generator and multiple discriminators. The upper  and the bottom framed parts correspond to the generator and multi-discriminator components, respectively. } %	\vspace{-0.3cm
	\label{fig-model} 
\end{figure*}

\subsection{Multi-Factor Generative Adversarial Network Framework}

Figure~\ref{fig-model} presents the overview of our proposed MFGAN framework for sequential recommendation.




\subsubsection{Basic Components} In this framework, we have two kinds of components undertaking different responsibilities for sequential recommendation:

(1) The upper component is the prediction component ($i.e.$ generator $G$) which is a sequential recommendation model and successively generates the next items based on the current historical sequence.
Note that the generator will not use any context information from the item side. It only makes the prediction conditioned on historical sequence data.

(2) The lower component is the evaluation component that is a set of $m$ discriminators $\{D_1, D_2, \dots, D_m\}$ for judging the rationality of generated sequences by using the information from multiple perspectives.
Each discriminator performs the judgement from a certain perspective based on the  information of some corresponding factor.
For example, in music recommender system, we may have multiple discriminators  specially designed with category information, popularity statistics, artist and album of music, respectively.



\subsubsection{Overall Procedure}  Following standard GAN~\cite{GAN-2014-NIPS},  the generator and multiple discriminators will play a min-max game.
At the $t$-step, the generator first generates a predicted item $\hat{i}_t$ based on the historical  sequence $\{ i_1, \dots, i_{t-1} \}$.
Then, 
each discriminator takes the $t$-length  sequence $\{ i_1, \dots, i_{t-1}, \hat{i}_t\}$ as the input and evaluates the rationality of the generated sequence using the information of some factor. The evaluation results are sent back to the generator to guide the learning of the generator at the next round.
Correspondingly, the discriminator is updated by taking the generated sequence and actual sequence~(\ie ground-truth user behaviors) as the training samples for improving its discriminative capacity.
As such, the two components force each other to improve in a mutual reinforcement way.
%As will be described later, both generators and discriminators are developed  on self-attention blocks, selectively attending the information from each position of user behaviors.% layer by layer.

\subsubsection{Merits} There are three major merits of using such a framework for sequential recommendation.
First, generally speaking, it is relatively difficult to train a capable generation-based sequential recommender using a direct optimization with a maximum likelihood loss (\eg exposure bias or data sparsity~\cite{Ranzato2015Sequence}). We utilize the discriminators to monitor the quality of the recommendation results of the generator, which are able to gradually improve the final recommendation performance. 
Second, it is more flexible to incorporate various kinds of factor information into  discriminators, so that the generator can  focus on the generation task itself.
Such a way is more resistible  to useless or noisy information from context data. It is easier to incorporate additional factors into an existing model. 
%Intuitively, not all the context information is useful at all time steps. 
%is relatively isolated with these information. and can focus on the generation task itself. 
 Third, instead of modeling all the factors in a discriminator, our framework decouples the effect of each factor by using multiple discriminators, which also improves the interpretability (\eg explaining why a special behavioral transition occurs) of the generated sequences.  




%The model structure of generators and discriminators are all built on self-attention blocks, selectively attending the information from each position of user behaviors layer by layer.
%Note that our proposed framework is general for current mainstream sequential recommendation methods, for simplicity, we illustrate it based on self-attention mechanism.
To instantiate the framework, we adopt the recently proposed self-attentive neural architecture~(\eg Transformer~\cite{transformer}) to develop the components of generator and discriminators, since it has been shown to be successful in various sequence-oriented tasks, including sequential recommendation~\cite{kang2018self}. While, it is flexible to implement our framework with other classes of models in practice.    
In the following sections, we will introduce the details of both components.

%will enable the generator to focus on the generation process, and contextual information can be  
%The core motivation is to use both generation and discrimination components 
%The major merits of using such a framework for sequential recommendation is in three folds. 

\ignore{Indeed, due to the flexibility of two components, it is much easier to add multiple factor information to the discriminators in our framework while it does not affect the generation on the generator side. 
At the same time, the discriminator side can decouple different factor information to interpret transition pattern of user behaviors.

}
\eat{
\subsection{The Generator}
\label{sec-generator}
As for sequential recommendation, previous works have proved the advantages of transformer on modeling user historical behaviors.
By adaptively assigning weights to previous items at each time step, it has achieved state-of-the-art performance.
Indeed, our proposed MFGAN is a general framework to support a variety of sequential models like recurrent neural network~\cite{GRU4Rec}, convolutional neural network~\cite{caser}, or transformer~\cite{kang2018self}.
For simplicity, we illustrate our generative model under the transformer structure.
The input embedding layer and the final prediction layer are also introduced here as follows.

\begin{figure*}[ht]
	\centering 
	\includegraphics[width=0.82\textwidth]{fig/model.pdf}
	\caption{The overview of the proposed MFGAN model with a generator and multiple discriminators. The upper part framed by the blue line is the generator and the lower part framed by the blue line contains multiple discriminators. } %	\vspace{-0.3cm
	\label{fig-model} 
\end{figure*}


\paratitle{Embedding Layer.}
Since the length of user's historical sequence is varied among users, we first take the fixed-length interaction sequence $L_u = \{ i_1, i_2, \cdots, i_n\}$ to calculate the historical preferences of user $u$, where $n$ denotes the maximum length that the model handles. If the length of an interaction sequence is less than $n$, we repeatedly add zero-padding to the left side of the sequence, otherwise we only keep the most recent sequence of length $n$.
We maintain an embedding matrix $M \in \mathbb{R}^{|\mathcal{I}| \times d}$ with the dimensionality of $d$ for the item vocabulary.
After stacking the input by the embedded representation from $M$, we get an input embedding matrix $E \in \mathbb{R}^{n \times d}$.
A learnable position encoding $P$ is also added to $E$ and supply the temporal information for the self-attention mechanism. Finally, the input of the generator is denoted by:
\begin{equation}
\begin{split}
    \label{eq-embedding}
    E_G = 
    \begin{bmatrix}
    E_1 + P_1\\
    E_2 + P_2 \\
    \vdots \\
    E_n + P_n
    \end{bmatrix}.
\end{split}
\end{equation}

\paratitle{Transformer Layer.}
A transformer block generally consists of two sub-layers, a multi-head self-attention sub-layer and a position-wise feed-forward network.
Multi-head self-attention mechanism has been proved the effectiveness on extracting the information selectively from different representation subspaces.
Thus, instead of attending information of user sequence by a single attention function, we adopt the multi-head self-attention mechanism for information extraction.
Specifically, multi-head attention is defined as below:
\begin{equation}
\label{eq-attention}
\begin{split}
MultiHeadAtt(F_l) &= [head_i;head_2;\dots,head_h]W^O \\
% head_i &= softmax(\frac{F_l W^Q_i (F_l W^K_i)^T}{\sqrt{d}_k})(F_l W^V_i
head_i &= Attention(F^l W^Q_i, F^l W^K_i, F^l W^V_i)
\end{split}
\end{equation}
where the $F^l$ is the input for the $l$-$th$ layer.
When $l=0$, $F^l$ is the original input $E_G$ of the generator.
The projection matrix $W^Q_i \in \mathbb{R}^{d \times d/h}, W^K_i \in \mathbb{R}^{d \times d/h}, W^V_i \in \mathbb{R}^{d \times d/h}$ and $W^O \in \mathbb{R}^{d \times d}$ are the corresponding learnable parameters for each attention head, $h$ is the head number.
The attention function is implemented by \textit{Scaled Dot-Product Attention}:
\begin{equation}
    Attention(\mathbf{Q}, \mathbf{K}, \mathbf{V}) = softmax(\frac{\mathbf{Q} \mathbf{K}^T}{\sqrt{d/h}})\mathbf{V}
\end{equation}
where $\mathbf{Q}$, $\mathbf{K}$, $\mathbf{V}$ represent query, key and value, respectively.
As in Equation~\eqref{eq-attention}, we adopt the choice $\mathbf{Q}=F_l W^Q_i,\mathbf{K}=F_l W^K_i,\mathbf{V}=F_l W^V_i$, which are the projections of the input embedding matrix $E_G$ and the representation of its upper layers.
The temperature $\sqrt{d / h}$ is the scale factor to avoid large values of the inner product.
Due to the nature of sequential recommendation that we could only utilize the information before the current time step,
we apply the triangle mask for the output of the multi-head self-attention function, forbidding all connections between $Q_i$ and $K_j$ ($j > i$).

Since the multi-head attention function is mainly based on the linear projections, we endow the non-linearity of the transformer structure by applying a followed point-wise feed-forward network.
The computation is defined as:
\begin{align}
    PFFN(F^l) &= [FFN(F^l_1)^T; \cdots; FFN(F_n^l)^T] \\
    FFN(x) &= \max(0, x W_1 + b_1) W_2 + b_2
\end{align}
where $W_1, b_1, W_2, b_2$ are the trainable parameters and not shared across layers.

\paratitle{Stacking Transformer Layer.}
The stacking of the transformer block is also applied.
As the model goes deep, it's usually beneficial to model more and more complex item-item interactions.
To alleviate the overfitting problem, we add residual connection~\cite{he2016deep} between each sub two layers intra the transformer structure, followed by layer normalization~\cite{layer_norm} and dropout operation~\cite{dropout}.

\paratitle{Prediction Layer.}
In the final layer of generator, we calculate the user’s preference for item $i$ through a dot product operation:
\begin{equation}
\begin{split}
    \label{eq-predict}
    y_{t, i}^u = F^L M_i^T,
\end{split}
\end{equation}
where $L$ is the number of transformer blocks and $M$ is the maintained item vocabulary matrix.
So far we can predict the target item using the user historical interaction sequence. 
We append the predicted item at the tail of the input sequence and constitute the fake sequence for discriminators.

Finally, we denote our entire generative model as $G_\theta$.
}

\subsection{The Generator Component}
\label{sec-generator}
In the MFGAN framework, let $G_\theta$ denote the generator component, parameterized by $\theta$, where $\theta$ denotes the set of all the related parameters in $G$.
We develop the  generator for sequential recommendation model by stacking the embedding layer, self-attention block, and the prediction layer to generate the target items. Next, we describe each part in detail.
%We illustrate them as follows:



\subsubsection{Embedding Layer} 
\label{embedding-layer}
We maintain an item embedding matrix $\bm{M}_G \in \mathbb{R}^{|\mathcal{I}| \times d}$ to project original one-hot representations of items to $d$-dimensional dense representations.
Given a $n$-length sequence of historical interactions, we apply a look-up operation from $\bm{M}_G$ to form the input embedding matrix $\bm{E} \in \mathbb{R}^{n \times d}$.
Furthermore, we incorporate a learnable position encoding matrix $\bm{P} \in \mathbb{R}^{n \times d}$ to enhance the input representations. 
In this way,  the input representations $\bm{E}_G \in \mathbb{R}^{n \times d}$ for the generator can be obtained by summing two embedding matrices:  $\bm{E}_G=\bm{E}+\bm{P}$.

\ignore{As for input user behaviors, we maintain an embedding matrix $M_G \in \mathbb{R}^{|\mathcal{I}| \times d}$ with the dimensionality of $d$ to project the high-dimensional one-hot representation of the item to low-dimensional dense representations.
After stacking the input by the embedded representation from $M_G$, we get an input embedding matrix $E \in \mathbb{R}^{n \times d}$.
A learnable position encoding $P$ is also added to $E$ and supply the temporal information for the self-attention mechanism. Finally, the input of the generator is denoted by:
\begin{equation}
\begin{split}
    \label{eq-embedding}
    E_G = 
    \begin{bmatrix}
    E_1 + P_1\\
    E_2 + P_2 \\
    \vdots \\
    E_n + P_n
    \end{bmatrix}.
\end{split}
\end{equation}
}

\subsubsection{Self-attention Block} Based on the embedding layer, we stack multiple self-attention blocks. 
A self-attention block generally consists of two sub-layers, a multi-head self-attention sub-layer and a point-wise feed-forward network.
Instead of attending information of user sequences with a single attention function,
multi-head self-attention mechanism has been adopted for effectively extracting the information  from different representation subspaces.
Specifically, multi-head self-attention is defined as below:

\begin{equation}
\label{eq-attention}
\begin{split}
\text{MultiHeadAtt}(\bm{F}^l) &= [head_i;head_2;\dots,head_h]\bm{W}^O, \\
% head_i &= softmax(\frac{F_l W^Q_i (F_l W^K_i)^T}{\sqrt{d}_k})(F_l W^V_i
head_i &= \text{Attention}(\bm{F}^l \bm{W}^Q_i, \bm{F}^l \bm{W}^K_i, \bm{F}^l \bm{W}^V_i),
\end{split}
\end{equation}
where the $\bm{F}^l$ is the input for the $l$-th layer.
When $l=0$, we set $\bm{F}^l$ to the input $\bm{E}_G$ of the generator.
Let $h$ denote the number of heads. 
The projection matrix $\bm{W}^Q_i \in \mathbb{R}^{d \times d/h}, \bm{W}^K_i \in \mathbb{R}^{d \times d/h}, \bm{W}^V_i \in \mathbb{R}^{d \times d/h}$ and $\bm{W}^O \in \mathbb{R}^{d \times d}$ are the corresponding learnable parameters for each attention head.
The attention function is implemented by scaled dot-product operation:

\begin{equation}
    \text{Attention}(\mathbf{Q}, \mathbf{K}, \mathbf{V}) = \text{softmax}(\frac{\mathbf{Q} \mathbf{K}^T}{\sqrt{d/h}})\mathbf{V},
\end{equation}
where $\mathbf{Q}=\bm{F}^l \bm{W}^Q_i,\mathbf{K}=\bm{F}^l \bm{W}^K_i$, and $\mathbf{V}=\bm{F}_l \bm{W}^V_i$, which are the linear transformations of the input embedding matrix.
The temperature $\sqrt{d / h}$ is the scale factor to avoid large values of the inner product.
In sequential recommendation, we can only utilize the information before  current time step, and we apply  the mask operation to the output of the multi-head self-attention function, removing  all connections between $\mathbf{Q}_i$ and $\mathbf{K}_j$ (for all cases of $j > i$).

As shown in Eq.~\eqref{eq-attention}, the multi-head attention function is mainly built on the linear projections.
We further endow the non-linearity of the self-attention block by applying a point-wise feed-forward network as:

\begin{align}
    \text{PFFN}(\bm{F}^l) &= [\text{FFN}(\bm{F}^l_1)^\top; \cdots; \text{FFN}(\bm{F}_n^l)^\top],\\
    \text{FFN}(\bm{x}) &= \max(0, \bm{x}\bm{W}_1 + \bm{b}_1) \bm{W}_2 + b_2,
\end{align}
where $\bm{W}_1, \bm{b}_1, \bm{W}_2, b_2$ are the trainable parameters and not shared across layers.

\eat{
The stacking of the transformer block is also applied.
As the model goes deep, it's usually beneficial to model more and more complex item-item interactions.
To alleviate the overfitting problem, we add residual connection~\cite{he2016deep} between each sub two layers intra the transformer structure, followed by layer normalization~\cite{layer_norm} and dropout operation~\cite{dropout}.
}

\subsubsection{Prediction Layer}

At the final layer  of the generator, we calculate the user's preference over the item set  through the softmax function:
\begin{equation}
\begin{split}
    \label{eq-predict}
    G_{\theta}(i_t | i_{1:t-1}) = \text{softmax}(\bm{F}_n^L \bm{M_G}^\top)_{[i_t]},
\end{split}
\end{equation}
where $L$ is the number of self-attention blocks and $\bm{M}_G$ is the maintained item embedding matrix defined in Section~\ref{embedding-layer}. 
%Here, we use the softmax function to generate the distribution of preditive probability for each item. 

%first take a dot product between $\bm{F}^L $

%$ \bm{y}_{G} \in \mathbb{R}^{|\mathcal{I}|}$ is the preference vector over the item set, and  $L$ is the number of transformer blocks and $\bm{M}_G$ is the maintained item embedding matrix defined in Section 3.2.1.
%The item with the highest prediction value in $\bm{y}_{G} $ is selected as the generated item for the generator.

\ignore{
In the final layer  of the generator, we calculate the user’s preference for items through a dot product operation.
\begin{equation}
\begin{split}
    \label{eq-predict}
    \bm{y}_{G} = \bm{F}^L \bm{M_G}^\top,
\end{split}
\end{equation}
where $ \bm{y}_{G} \in \mathbb{R}^{|\mathcal{I}|}$ is the preference vector over the item set, and  $L$ is the number of transformer blocks and $\bm{M}_G$ is the maintained item embedding matrix defined in Section 3.2.1.
The item with the highest prediction value in $\bm{y}_{G} $ is selected as the generated item for the generator.
}
%We further append it at the tail of the input sequence and constitute the fake sequence for discriminators.

\subsection{Factor-specific Discriminator Components}
As mentioned before, we consider $m$ kinds of factor information that is useful to improve the sequential recommendation. Instead of directly feeding them into the generator, we set a unique discriminator for each factor, such that various kinds of context information  can be utilized and decoupled via the factor-specific discriminators. 

Specially, we have $m$ discriminators $D_\Phi = \{ D_{\phi_1}, D_{\phi_2}, \dots, D_{\phi_m} \}$, in which the $j$-th discriminator is parameterized by $\phi_j$.
The function of each discriminator is to determine whether the generated recommendation sequence by the generator is rational or not. This is cast as a binary classification task, \ie discriminating between generated or actual recommendation sequence. 
We assume that different discriminators are equipped with different parameters and work independently. 

\ignore{As for discriminator, we propose a multiple $\Phi$-parameterized discriminative model $D_\Phi = \{ D_{\phi_1}, D_{\phi_2}, \dots, D_{\phi_m} \}$ to provide a multi-perspective guidance for improving generator $G_\theta$. 
The purpose of a single discriminator is to determine if a given sequence is reasonable or not from the corresponding factor information.
Different discriminators work independently and do not share parameters.
}



\ignore{Specifically, each discriminator is designed for a binary classification task built on self-attention blocks. 
Since the task of the discriminator is much easier than that of the generator, we have a simplified architecture of the discriminator with only one self-attention block to prevent the discriminator from being too critical and further affecting the training process of the generator.
}

\subsubsection{Embedding Layer} Considering a specific discriminator $D_{\phi_j}$,  we first construct an  input embedding matrix $\bm{E}_{D}^{j}\in \mathbb{R}^{n\times d}$ for a $n$-length sequence by summing the factor-specific embedding matrix $\bm{C}^{j}$ and the positional encoding matrix $\bm{P}$, namely $\bm{E}_{D}^{j} = \bm{C}^{j}+\bm{P}$. %Here, $\bm{C}^{i}$ denotes the embedding representations of the sequence with  
To construct the  $\bm{C}^{j}$, we adopt a simple yet effective method: first discretize the possible values of a factor into several bins,  then set a unique embedding vector for each bin, and finally derive $\bm{C}^{j}$ using a look-up operation by concatenating the embeddings for the bin IDs from the input sequence.  

 %sequences corresponding to a specific factor from it's own vocabulary $M_{D}^i$.
%The position embedding is added to the input representation and we constitute the input matrix $E_{D}^i$ for each discriminator.
\subsubsection{Architecture}  To develop the discriminator, we adopt the similar architecture of the generator. In our framework, the generator predicts the recommended sequence, and the discriminators are mainly used to improve the generator. 
Hence, we adopt a relatively weak architecture with only one self-attention block for avoiding the case that the discriminator is too strong and cannot send suitable feedback to the generator. 
The one-layer self-attention block is computed as:

\begin{align}
    % \small
    \label{eq-sa-d}
    \bm{A}^{j} &= \text{MultiHeadAtt}(\bm{E}_{D}^{j}), \\
    \bm{H}^{j} &= \text{PFFN}(\bm{A}^{j}).
\end{align}
Note that unlike the generator, the self-attention block of the discriminator can refer to the information of subsequent positions when trained at the $t$-th position.
Hence,  the discriminator adopts a \emph{bi-directional} architecture by removing the mask operation. In this way, the discriminator can model the interaction between any two positions, and make a more accurate judgement by considering the overall sequential characteristics. 
While, the generator does not utilize such bi-directional sequential characteristics. 
As such, 
the discriminator is expected to provide additional supervision signals, though it shares the similar architecture with the generator. 

%While, such bi-directional sequential characteristics cannot be utilized in the generator, so that the discriminator is expected to provide additional supervision signals although they s
%It is also a key step to make the discriminator capture more information compared with  


\ignore{Note that unlike the generator, the self-attention block in discriminator can consider the subsequent positions when training the $t$-$th$ position, because the task of the discriminator is no longer to predict the current position based on the previous positions, but to judge the rationality throughout the sequence.
We remove the mask operation for each discriminator and keep the interactions between any two positions.}
% We also adopt residual connections, layer normalization and dropout operation to avoid overfitting problem.

Finally, the  degree of the rationality  for the generated recommendation sequence is measured by a  Multiple-Layer Perceptron~(MLP):

\begin{equation}\label{eq-mlp}
    % \small
    \hat{y}_{j} = \text{MLP}(\bm{H}_n^j),
\end{equation}
where $\hat{y}_{j}$ is the predicted degree of the rationality from the the  MLP component based on 
 the output of the self-attention block $\bm{H}^j$.
A  rationality score reflects the probability that a sequence is from actual data distribution judged by some discriminator. 

Since we have $m$ discriminators  \emph{w.r.t.} different factors, we can obtain a set of predicted rationality scores $\{ \hat{y}_{1}, \hat{y}_{2}, \dots, \hat{y}_{m} \}$. 
As will be illustrated later, these rationality scores can be used for supervision signals to guide the learning of the generator.
%$\varphi$ is the non-linearity activation function. $W_l$ and $b_l$ are the corresponding parameters of the $l$-th layer.
%The prediction signals $\{ \hat{y}_{1}, \hat{y}_{2}, \dots, \hat{y}_{m} \}$ from all discriminators also serve as the rewards for the guidance of generator training.
%We illustrate the details in the next section.

\subsection{Multi-adversarial Training}
As described previously, there is  one generator $G_\theta$ and multiple discriminators $D_\Phi = \{ D_{\phi_1}, D_{\phi_2}, \dots, D_{\phi_n} \}$. The generator $G_\theta$ successively predicts the next item based on historical sequence data, and the discriminators try to discriminate between the predicted sequence and the actual sequence.  In this part, we present the multi-adversarial training algorithm for our approach. 

\ignore{
As illustrated in previous subsection, we have one generative model 
$G_\theta$ and multiple discriminator $D_\Phi = \{ D_{\phi_1}, D_{\phi_2}, \dots, D_{\phi_n} \}$.
Generator $G_\theta$ successively generates the next item based on user historical sequence $I = \{ i_1, \dots, i_{T-1}\}$ and correspondingly yield the following items $I = \{ i_2, \dots, i_T\}$ at each time step.
Multi-discriminator $D_\Phi$ can determine whether the sequence generated by the generator is a reasonable sequence or not from multiple perspectives with different factors.
}

\subsubsection{RL-based Formalization} Because sampling from the item set is a discrete process,  gradient descent cannot be directly applied to solve the original GAN formulation for our recommendation task. 
As such, following~\cite{Yu2017SeqGAN},  we first formalize the sequential recommendation task in a reinforcement learning~(RL) setting. At the $t$-step, the \emph{state} $s$ is represented by the previously recommended sub-sequence  $i_{1:t-1}=\{ i_1, i_2, \dots, i_{t-1} \}$; the \emph{action} $a$ is to select the next item $i_t$ for recommendation, controlled by a \emph{policy} $\pi$ that is defined according to the generator: $\pi(a=i_t | s)=G_\theta(i_t| i_{1:t-1})$; when an action is taken, it will transit from $s_t$  to a new state $s'$, corresponding to the  sub-sequence  $i_{1:t}=\{ i_1, i_2, \dots, i_{t} \}$;  taking an action  will lead to some \emph{reward} $r$. The key point is that we utilize the discriminator components to provide the reward signal for guiding the learning of the generator. We define the expected return $Q(s,a)$ for a pair of state and action, namely the $Q$-function, as below

\begin{equation}
%\begin{split}
% \small
\label{eq:action-value}
Q(s = i_{1:t-1}, a = i_t) = \sum_{j=1}^{m} \omega_j \hat{y}_j, 
\end{equation}
where $\hat{y}_j$ is the rationality score~(Eq.~\eqref{eq-mlp}) of current sequence according to the $j$-th discriminator, and $\omega_j$ is the combination coefficient defined through a $\lambda$-parameterized softmax function: 
\begin{equation}\label{eq-lambda}
\omega_j = \frac{\exp(\lambda\hat{y}_j)}{\sum_{j'=1}^m \exp(\lambda\hat{y}_{j'})},
\end{equation}
where $\lambda$ is a tuning parameter that will be discussed later.

As the discriminator is updated iteratively, it  gradually pushes the generator to its limit, which will generate more realistic recommended items.  Through multiple-factor enhanced architecture, the generator can obtain guidance of sequential characteristics in the interaction sequence from different perspectives.


%$\omega_j = {\exp{(\lambda D_{\phi_j} (I_{1:T}))}} / {\sum_{k} \exp{(\lambda D_{\phi_k} (I_{1:T})})}$ is the weight for the j-$th$ discriminator and $|\Phi|$ is the number of discriminators.
 

%Instead of directly giving the reward of individual steps, we define the $Q$ function that computes 
 


\ignore{ and set to the mean of the predicted scores from all the discriminators:
\begin{equation}
r = \text{Average}(\{ \hat{y}_{1}, \hat{y}_{2}, \dots, \hat{y}_{m} \}),
\end{equation}
where $\hat{y}_{i}$ is defined in Eq.~\eqref{eq-mlp} reflecting the confidence level of being an actual sequence by the $i$-th discriminator. 
}


\ignore{
As sampling the recommended item is a discrete process, it can not be directly applied by gradient descent as the original GAN formulation for our recommendation task.
As such, following~\cite{Yu2017SeqGAN}, we interpret our sequential recommendation task based on reinforcement learning.
In timestamp $T$, the state $s$ is represented by the current produced sub-sequence of items $I_{1:T-1}=\{ i_1, i_2, \dots, i_{T-1} \}$.
The action $a$ is the next generated item $i_t$ to select.
Since the output of the generator $G_\theta = P(i_T|I_{1:T-1})$ is a probability distribution over item vocabulary, the policy is stochastic in our problem.
The transition probability $P$ is deterministic.
After the action has been chosen, $p^a_{s, s'}$ is equal to 1 for the next state $s'=I_{1:t}$ if the current state is $s=I_{1:T-1}$ and the action is $a=i_T$.
The reward $R$ is propagated from the multi-discriminator, measuring the rationality of the generated sub-sequence from multiple perspectives.
}
\eat{
From the previous subsection, we have the generative model $G_\theta$ and the multi-discriminator $D_\Phi = \{ D_{\phi_1}, D_{\phi_2}, \dots, D_{\phi_n} \}$.
Generator $G_\theta$ can predict the next item $i_T$ of user historical sequence $I = \{ i_1, i_2, \dots, i_{T-1}\}$ and equivalent to produce a generative sequence $I = \{ i_1, i_2, \dots, i_T\}$. Multi-discriminator $D_\Phi$ can determine whether the sequence generated by the generator is a reasonable sequence from multiple perspectives with different factors.

The main problem during training is that the sequence obtained by the generator $G_\theta$ is discrete, and GAN does not work well with discrete data. Most of the current optimization methods are based on gradients, in the situation of discrete data, the discriminators cannot feed the gradient back to the generator. 
To solve this problem, following~\cite{Yu2017SeqGAN}, we interpret the sequential recommendation task based on reinforcement learning. 

During the training process of the generator, each predicted item will form a generated sequence with the historical interaction sequence, and then obtain a reward from the discriminators, representing the rationality of the generated sequence.

For each input sequence, at timestamp $T-1$, we have the historical interaction sequence $I_{1:T-1}$. We consider the prediction of the next item as a policy.
}


\subsubsection{Learning Algorithm} After the task is formulated as a RL setting,  we can apply the classic policy gradient to learn the model parameters of the generator. Formally, the objective of the generator $G_\theta(i_t|i_{1:t-1})$ is to maximize the expected reward at the $t$-th step:
\begin{equation*}
\begin{split}
\mathcal{J}(\theta) = \mathbb{E}[R_t|i_{1:t-1}; \theta] = \sum_{i_t \in \mathcal{I}} G_\theta(i_t|i_{1:t-1}) \cdot Q(i_{1:t-1}, i_t),
\end{split}
\end{equation*} 
where $G_\theta(i_t|i_{1:t-1})$  and $Q(i_{1:t-1}, i_t)$ are defined in Eq.~\eqref{eq-predict} and Eq.~\eqref{eq:action-value}, respectively. 
$R_t$ denotes the reward of a generated sequence.
The gradient of the objective function $\mathcal{J}(\theta)$ \emph{w.r.t.} the generator's parameters $\theta$ can be derived as:
\begin{equation}
% \small
\label{eq:gradient}
\begin{split}
\nabla_\theta \mathcal{J}(\theta) 
%&= \mathbb{E}_{i_{1:t-1}} [\sum_{i_t \in \mathcal{I}} \nabla_\theta G_\theta(i_t|i_{1:t-1}) \cdot Q(i_{1:t-1}, i_t)]\\
&= \nabla_\theta \sum_{i_t \in \mathcal{I}} G_\theta(i_t|i_{1:t-1}) \cdot Q(i_{1:t-1}, i_t)\\
&= \sum_{i_t \in \mathcal{I}} \nabla_\theta G_\theta(i_t|i_{1:t-1}) \cdot Q(i_{1:t-1}, i_t)\\
&= \sum_{i_t \in \mathcal{I}} G_\theta(i_t|i_{1:t-1}) \nabla_\theta \log G_\theta(i_t|i_{1:t-1}) \cdot Q(i_{1:t-1}, i_t) \\
&= \mathbb{E}_{i_t \sim G_\theta(i_t|i_{1:t-1})}[\nabla_\theta \log G_\theta(i_t|i_{1:t-1}) \cdot Q(i_{1:t-1}, i_t)].
\end{split}
\end{equation} 


We update the  parameters of the generator using gradient ascent as follows:
\begin{equation}
\begin{split}
\label{E2}
\theta \leftarrow \theta + \gamma \nabla_\theta \mathcal{J}(\theta),
\end{split}
\end{equation}
where $\gamma$ is the step size of the parameter update.


\ignore{$R_t$ is the reward for a complete sequence generated by generator. As mentioned before, the reward is from the discriminators $D_\Phi$ and denoted by action-value function $Q_{D, G}(s, a)$ of the sequence, measuring the expected value signal based on the state $s$ and action $a$.
Indeed, we take the estimated probability of being a reasonable sequence from multiple discriminators as the reward:
\begin{equation}
\begin{split}
\label{eq:action-value}
Q_{D,G}(a = I_{1:T-1}, s = i_T) 
&= softmax(D_{\Phi} (I_{1:T}), \lambda) \\
&= \sum_{j=1}^{|\Phi|} \omega_j D_{\phi_j} (I_{1:T}),
% &= \frac{\sum_{j=1}^{|\Phi|} D_{\phi_j} (I_{1:T})}{|\Phi|},
\end{split}
\end{equation}
where $\omega_j = {\exp{(\lambda D_{\phi_j} (I_{1:T}))}} / {\sum_{k} \exp{(\lambda D_{\phi_k} (I_{1:T})})}$ is the weight for the j-$th$ discriminator and $|\Phi|$ is the number of discriminators.
To simplify the notation, we use $\alpha_j$ to indicate $D_{\phi_j} (I_{1:T})$ and $\alpha$ to indicate $Q_{D,G}(s = I_{1:T-1}, a = i_T)$ in Fig.~\ref{fig-model}.
}

After updating the generator, we continue to optimize  each discriminator $D_{\phi_j}$ by minimizing the following objective loss:
\begin{equation}
\label{eq:opt_d}
\begin{split}
\min \limits_{\phi_j} - \mathbb{E}_{i_{1:t} \sim P_{\text{data}}}[\log D_{\phi_j} (i_{1:t})] - \mathbb{E}_{i_{1:t} \sim G_\theta}[\log (1 - D_{\phi_j} (i_{1:t})]\},
\end{split}
\end{equation}
where $P_\text{data}$ is the real data distribution.
%Such an optimization is performed by following the standard GD algorithm. 
% We implement the model by \emph{Tensorflow} with the \emph{Adam} optimizer in mini batches.

Algorithm~\ref{alg1} presents the details of the training algorithm for our approach.
%We perform a min-max game between the generator and the discriminator.
The parameters of $G_{\theta}$ and multiple discriminators $D_{\Phi}$ are pretrained correspondingly. 
% initialized by pretraining the model under different tasks.
For each $G$-step, we generate the recommended item based on  the previous sequence $i_{1:t-1}$, and then update the parameter by policy gradient with the reward provided from multiple discriminators.
For each $D$-step, the recommended sequence is considered as the negative samples and we take the actual sequence from training data as positive ones.
Then the discriminators are updated to discriminate between positive and negative sequences accordingly.
Such a process is repeated until the algorithm converges.

\begin{algorithm}[t] %算法开始 
\caption{The learning algorithm  for our MFGAN framework.} %算法的题目 
\label{alg1} %算法的标签 
\begin{algorithmic}[1] %此处的[1]控制一下算法中的每句前面都有标号 
\REQUIRE generator $G_\theta$; discriminators $D_\Phi = \{D_{\phi_1} ,  \dots, D_{\phi_{m}}\}$; user-item interactive sequence dataset $\mathcal{S}$ %输入条件(此处的REQUIRE默认关键字为Require，在上面已自定义为Input)  %输出结果(此处的ENSURE默认关键字为Ensure在上面已自定义为Output) 
\STATE Initialize $G_\theta$, $D_\Phi$ with random weights $\theta$, $\Phi$
\STATE Pre-train $G_\theta$ using MLE
\STATE Generate negative samples using $G_\theta$ for training $D_\Phi$
\STATE Pre-train $D_\Phi$ via minimizing cross-entropy
% repeat-until loop 
\REPEAT 
    % for loop 
    \FOR{$G$-steps} 
        \STATE Generate the predicted item $i_t$ using $i_{1:t-1}$
        \STATE Obtain the generated sequence $i_{1:t}$
        \STATE Compute $Q(s = i_{1:t-1}, a = i_t)$ by Eq.~ \eqref{eq:action-value}
        \STATE Update generator parameters $\theta$ via policy gradient Eq.~ \eqref{E2}
    \ENDFOR 
    
    \FOR{$D$-steps} 
    \STATE Use $G_\theta$ to generate negative examples
   % \STATE Retrieve the corresponding sequences on each factor of the original sequence for the discriminator
    \STATE Train $m$ discriminators $D_\Phi$ by Eq.~\eqref{eq:opt_d}
    \ENDFOR 
\UNTIL{Convergence} 

\end{algorithmic} 
\end{algorithm}

\subsection{Discussion and Analysis}\label{sec:theory}

% As such, the min-max game is designed to optimize:
% \begin{equation}
% \begin{split}
%     J^{G*, D*} = \min_{\theta} \max_{\phi} \sum_{i=1}^N (\mathbb{E}_{d \sim p_{true}(i_T|I_{1:T-1})}[log(D_{\Phi}(I_{1:T}))] \\ + \mathbb{E}_{d \sim p_{\theta}(i_T|I_{1:T-1})}[log(D_{\Phi}(I_{1:T}))])
% \end{split}
% \end{equation}


In this section, we analyze the effectiveness and the stability of the multi-adversarial architecture in our task.

As mentioned before, we train the MFGAN model in an RL way by policy gradient. Since we have multiple discriminators, from each discriminator we receive a reward to guide the training process of the generator. 
Recall that we use a $\lambda$-parameterized softmax function to combine the reward signals from multiple discriminators in Eq.~\eqref{eq-lambda}. By using such a parameterization, our reward function can be implemented in several  forms: 

%Now, we discuss the effect of various integration methods on our learning algorithm.
(1)  $\lambda\rightarrow -\infty$: it selects the discriminator with the minimum reward, \ie \emph{min};

(2)  $\lambda\rightarrow +\infty$: it selects the discriminator with the maximum reward, \ie \emph{max};

(3) $\lambda=0$: it becomes a simple average over all the discriminators, \ie \emph{mean}; 

(4) Others: it adopts a ``soft'' combination of multiple reward values. 
%How to use these rewards to guarantee effective and stably training of the generator is a problem.

Among the four cases, we first study two extreme strategies, namely \emph{max} and \emph{min}.
As shown in \cite{ICLR17GMAN}, it is too harsh for the generator by adopting the minimum reward from the  discriminators.
  Let $p_G (x)$ denote the distribution induced by the generator. The low reward only indicates the position where to decrease $p_G (x)$, and does not specifically indicate the position where to increase $p_G (x)$. In addition, decreasing $p_G (x)$ will increase $p_G (x)$ in other regions of distribution space $\mathcal{X}$ ( keeping $\int_\mathcal{X} p_G (x) = 1$), and the correctness of this region cannot be guaranteed. Hence, the \emph{min} strategy is not good to train our approach. Conversely, \emph{max} always selects the maximum reward that is able to alleviate the above training issue of \emph{min}. However, since multiple factors are involved in the discriminators, some ``prominent'' factor will dominate the learning process, leading to insufficient training of other factors.
%For example,  for music recommendation, if the factor of \emph{artist} is more significant to be correlated with users' behaviors than other factors,  the discriminators \emph{w.r.t.} other factors might not be  well trained since their signals are often \emph{hidden} by the prominent discriminator.


\ignore{Following~\cite{ICLR17GMAN}, an intuitive way is to select the harshest discriminator to signal the generator, $i.e.$, adopt the min reward among all the discriminators, but the trouble is that it is too harsh a critic. In practice, training against a far superior discriminator can impede the generator’s learning.
This is because the sequential recommendation task is more difficult than the discrimination task, thus the generator is unlikely to generate samples that the discriminator considers reasonable, so the generator will always receive low reward. Let $p_G (x)$ denote the distribution induced by the generator. The low reward only indicates the position where to decrease $p_G (x)$, and does not specifically indicate the position where to increase $p_G (x)$. In addition, decreasing $p_G (x)$ will increase $p_G (x)$ in other regions of $\mathcal{X}$ ( keeping $\int_\mathcal{X} p_G (x) = 1$), and the correctness of this region cannot be guaranteed. Conversely, if the discriminator is lenient, the generator may get high reward on higher quality samples, which may better guide the generator to gather $p_G (x)$ in approximately correct region of $\mathcal{X}$. 
}
\ignore{
As a result, we adopt the softmax operator instead of min operator to make use of the rewards of multiple discriminators:
\begin{equation}
\begin{split}
\label{eq:action-value}
softmax(D_{\Phi}, \lambda) = \sum_{j=1}^{|\Phi|} \omega_j D_{\phi_j},
% &= \frac{\sum_{j=1}^{|\Phi|} D_{\phi_j} (I_{1:T})}{|\Phi|},
\end{split}
\end{equation}
where $\omega_j = {\exp{(\lambda D_{\phi_j})}} / {\sum_{k} \exp{(\lambda D_{\phi_k} })}$ is the weight for the $j$-$th$ discriminator.
To increase the odds of providing constructive feedback to the generator, we set $\lambda$ to zero to apply the mean option. Combined with the calculation of reward, we can rewrite the training objective of the generator as:
\begin{equation*}
\begin{split}
J(\theta) = \frac{1}{|\Phi|} \sum_{i_T \in \mathcal{I}} [G_\theta  \sum_{j=1}^{|\Phi|} D_{\phi_j}].
\end{split}
\end{equation*}
} 

Compared with the former two cases, the latter two cases seem to be more reasonable in practice. 
They consider  the contributions from all the discriminators. 
Specially, we can have an interesting observation: the gradient $\nabla_\theta \mathcal{J}(\theta)$ of the generator calculated in Eq.~\eqref{eq:gradient} is more robust for model learning  due to the use of multiple discriminators. The major reason is that the $Q$-function in Eq.~\eqref{eq:action-value} is 
equal to zero \emph{if and only if}  $D_{\phi_j} = 0$ for all $j$, when all the discriminators give zero  reward.
Therefore, using multiple discriminators is indeed useful to stabilize the learning process of our approach. 
%Another merit is that we can model the information of various factors in multiple discriminators, and such a way is able to enhance the interpretability of the generator, \eg the reward values can be treated as the importance of various context information at each step.   
In our experiments, we do not observe a significant difference between the last cases on our task. 
Hence, we adopt the simpler \emph{mean} way to set our reward function.

Our work is closely related to general sequence prediction studies with adversarial training~\cite{Yu2017SeqGAN} or reinforcement learning~\cite{Ranzato2015Sequence}.  Similar to SeqGAN~\cite{Yu2017SeqGAN}, we set up two  components with different roles of \emph{generator} and \emph{discriminator}, respectively. 
Also, it is  easy to make an analogy between the two roles and the concepts of ``\emph{actor}'' and ``\emph{critic}'' in the actor-critic algorithm in RL~\cite{Ranzato2015Sequence}.
%With such two different components, it is more flexible to decouple useful information for achieving different modeling purposes in sequential recommendation. 
Compared with previous sequential recommendation models~\cite{GRU-f,HuangWSDM19, li2019review}, 
our approach takes a novel perspective that decouples various factors from the prediction component. 
%It is more flexible to achieve this purpose with two different components. 
In our model, each discriminator has been fed with the information of some specific factor.
Such a way is able to enhance the interpretability of the generator, that is to say,  the reward values of discriminators can be treated as the importance of influencing factors at each time step.   
%In this way, our work makes an important difference to prior 
With the proposed framework, we believe there is much room to consider more advanced implementations or functions for generator and discriminators for improving sequential recommendation. 


%While, our work is the first time that adversarial training has been applied in sequential recommendation. 

%Different from prior studies~\cite{}, our focus is to decouple factor utilization from the sequence prediction component.   e would like to keep the prediction component more 

%Such an idea is also similar to the analogy of ``\emph{actor}'' and ``\emph{critic}'' in RL~\cite{}.

\ignore{Note that the gradient $\nabla_\theta J(\theta)$ of the generator calculating in Eq.~\eqref{eq:gradient} is minimized at $\sum_{j=1}^{|\Phi|} D_{\phi_j} = 0$, if and only if $D_{\phi_j} = 0$ for all $j$. So generator only receives a vanishing gradient when all $D_{\phi_j}$ consider that the sample is unreasonable. For our multiple discriminators from different perspectives, the probability of occurrence is much smaller than the single discriminator without external factors. In other wards, the generator only needs to fool a single $D_{\phi_j}$ to receive a constructive feedback. This result allows the generator to successfully minimize the generator objective and generally guarantee the stability of the training process. We also verified the above conclusions in further experiments.
}

==> Sequential Recommendation with Self-Attentive Multi-Adversarial Network/subfile2/4_exp.tex <==
\section{Experiments}
\label{sec:exp}
In this section, we first setup the experiments,  then report major comparison results and other detailed analysis. 

\subsection{Dataset Construction}
We construct experiments on three public datasets from different domains, including \textsc{MovieLens-1M} movie~\cite{Movielens}, \textsc{Yahoo!} music\footnote{\url{https://webscope.sandbox.yahoo.com/catalog.php?datatype=r}.} and \textsc{Steam}~\cite{kang2018self} game. 
Since the \textsc{Yahoo!} dataset is very large, we randomly sample a subset of ten thousand users from the entire dataset. 
We group the interaction records by users, sort them by the timestamps ascendingly, and form the interaction sequence for each user.
Following \cite{RendleFS10}, we only keep the $k$-core dataset, filtering out unpopular items and inactive users with interaction records which are fewer than $k$. We set $k = 5, 10, 5$ for the \textsc{MovieLens-1M}, \textsc{Yahoo!} and \textsc{Steam} datasets, respectively. 

%in the game dataset, $k = 10$ in the music dataset and $k = 5$ for the movielens-1m datasets. 
The three datasets contain several kinds of context information. We extract such context information as \emph{factors}:

 (1) For \textsc{MovieLens-1M} dataset, we select category, popularity, and knowledge graph information as factors. Note that we treat the knowledge base~(KB) information as a single factor, since we would like to develop a strong factor. 
We use the KB4Rec dataset~\cite{KB4Rec} to obtain \emph{item-to-entity} alignment mapping, and then obtain the KB information from \textsc{Freebase}~\cite{freebase}. We adopt the classic TransE~\cite{transe-NIPS-2013} to learn the factor representation for KB information. 

(2) For \textsc{Yahoo!} dataset, we select category, popularity, artist and album as factors. 

(3) For \textsc{Steam} dataset, we select category, popularity, price and developer as factors. 
\ignore{For the numeric factors like price, we divide all prices into multiple ranges and use it to indicate the price level.}

Note that for all the three datasets, we have incorporated a special kind of factor, \ie item ID. Although it has been utilized in the generator, it can be utilized by the discriminator in a different way, \ie using a bi-directional Transformer architecture. 
Item ID can be used as a reference to compare the usefulness of the other kinds of factor information. 
Following~\cite{kang2018self}, we split each user interaction sequence into three parts:  the last item in the interaction sequence is treated as test data, the item just before the last is used for validation and the rest data is considered  as  training data.
The statistics of three datasets after preprocessing are summarized in Table~\ref{tab-data}.


\ignore{Each dataset has its own factors, in movielens-1m datasets, we leverage category, popularity, and knowledge graph information, in music dataset we leverage category, popularity, artist and album, and we utilize category, popularity, price and developer in the game dataset. We also treat origin identifier of item as a factor which is not external context information.
As we adopt knowledge graph information as a factor in movielens-1m dataset, we link the filtered items with \textsc{Freebase}~\cite{freebase} entities using KB4Rec dataset~\cite{KB4Rec}, which contains the alignment records between Freebase entities and items from several domains. We only keep the interactions related to the linked items in the final dataset and we apply TransE~\cite{transe-NIPS-2013} to obtain the entity embeddings from knowledge graph. To train TransE algorithm, we start with linked entities as seeds and expand the graph with one-step search.}

\begin{table}[htbp]
  \centering
  \caption{Statistics of the three datasets.}
  \label{tab-data}%
    \begin{tabular}{c r r r r}
		\hline
		Dataset & \#Users & \#Items & \#Interactions & \#Factors\\
		\hline
		\hline
		Movielens-1m   & 6,040 	& 3,361     & 996,834   & 4\\
		Music   & 10,000     & 136,630   & 3,732,463 & 5\\
% 		Tmall   & 44249     & 30,927    & 1,065,601 & 4\\
		Game   & 51,995 	& 12,037    & 1,789,953 & 5\\
		\hline

    \end{tabular}%
\end{table}%



\begin{table*}[h]
	\centering
	\caption{Performance comparison of different methods for sequential recommendation task on three datasets. We use bold and underline fonts to denote the best performance and second best performance method in each metric respectively.}
	\label{tab:results-all}%
	\begin{tabular}{| p{1.3cm} | p{1.3cm}<{\centering} p{1.3cm}<{\centering} p{1.3cm}<{\centering}| p{1.3cm}<{\centering} p{1.3cm}<{\centering} p{1.3cm}<{\centering}| p{1.3cm}<{\centering} p{1.3cm}<{\centering} p{1.3cm}<{\centering}|}
		\hline
		\multirow{2}{*}{Models}&\multicolumn{3}{c|}{Movie}&\multicolumn{3}{c|}{Music}&\multicolumn{3}{c|}{Game}\\
		\cline{2-10}
		&NDCG@10    & HR@10 & MRR&NDCG@10    & HR@10 & MRR&NDCG@10    & HR@10 & MRR\\
		\hline
		\hline
		PopRec  & 0.2290 & 0.4200 & 0.1940 & 0.3984 & 0.6322 & 0.3408 & 0.4129 & 0.6738 & 0.3477\\
		BPR     & 0.3063 & 0.5576 & 0.2505 & 0.4538 & 0.6695 & 0.3992 & 0.4203 & 0.6919 & 0.3511\\
		FM      & 0.1935 & 0.3522 & 0.1690 & 0.2196 & 0.4165 & 0.1812 & 0.1383 & 0.2818 & 0.1216\\
		IRGAN   & 0.2263 & 0.4201 & 0.1903 & 0.2857 & 0.5120 & 0.2332 & 0.3942 & 0.6525 & 0.3307 \\
		\hline
		FPMC 	& 0.3754 & 0.5990 & 0.3237 & 0.4330 & 0.5768 & 0.4022 & 0.3699 & 0.6167 & 0.3107\\
		GRU 	& 0.4014 & 0.6233 & 0.3763 & 0.4843 & 0.7778 & 0.4053 & 0.2383 & 0.4212 & 0.2037\\
		GRU$_F$ & 0.4130 & 0.6409 & 0.3552 & 0.5470 & 0.8112 & 0.3961 & 0.2806 & 0.4860 & 0.2369 \\
		SASRec  & \underline{0.5849} & \underline{0.8132} & \underline{0.5214} & \underline{0.8356} & \underline{0.9293} & \underline{0.8074} & \underline{0.5895} & \underline{0.8351} & \underline{0.5203} \\
		\hline
		%SFGAN  & 0.6032 & 0.8212 & 0.5423 & 0.8478 & 0.9353 & 0.8207 & 0.5990 & 0.8426 & 0.5308 \\
		MFGAN & \textbf{0.6185} & \textbf{0.8318} & \textbf{0.5587} & \textbf{0.8556} & \textbf{0.9417} & \textbf{0.8286} & \textbf{0.6035} & \textbf{0.8488} & \textbf{0.5346} \\
		\hline
	\end{tabular}%
\end{table*}%	

\subsection{Experimental Settings}

\subsubsection{Evaluation Protocol}
To assess whether our method can improve the sequential recommendation, we adopt a variety of evaluation metrics widely used in previous works~\cite{RendleFS10, Huang-2018-SIGIR, HuangWSDM19}: Mean Reciprocal Rank (MRR), top-$k$ Normalized Discounted cumulative gain (NDCG@10) and Hit Ratio (HR@10). 
%To avoid heavy computation on all user-item pairs, we followed the strategy in \cite{kang2018self}. For each user $u$, we randomly sample 100 negative items, and rank these items with the ground-truth item. The evaluation metrics can be evaluated according to the rankings of these items. We report the average score for all test users.
%Following previous works on sequential recommendation~\cite{kang2018self, RendleFS10, Huang-2018-SIGIR}, we consider the evaluation task for next item recommendation. We hold out the last item of the interaction sequence as the test data, the item just before the last has been treated as the validation data. 
Since the item set is large, it is time-consuming to enumerate all the items as candidate. For each positive item in the test set, we pair it with 100 sampled items that the user has not interacted with as negative items. The evaluation metrics can be computed according to the rankings of these items. 
We report the average score over all test users.


\subsubsection{Implementation Details}
For our proposed MFGAN, we use two self-attention blocks in the generator and one self-attention block in discriminators. In both generator and discriminators, item embeddings are shared in embedding layer and prediction layer. We implement MFGAN with \emph{Tensorflow}, and use \emph{Adam} optimizer. At the pre-training stage, we first train the generator and discriminators to converge separately. At the adversarial training stage, we alternatively train the generator and discriminators with 100 epochs and 1 epoch, respectively. The learning rates   are set to 0.001 for \textsc{MovieLens-1M} dataset, and 0.0002 for \textsc{Steam} and \textsc{Yahoo!} datasets, and the dropout rates are all set to 0.2 for the three datasets.
For each factor, we discretize its possible values into several bins if needed. Each bin is associated with an embedding vector. 
%We adopt a discretization method to all the factors by splitting the vale range into several possible bins. 
The item embedding size and all the factor embedding sizes are set to 50, the KB embedding size with \textsc{TransE} is set to 100.
The mini-batch sizes are set to 128 in generator and 16 in discriminators.

%\textsc{MovieLens-1M}, \textsc{Yahoo!} and \textsc{Steam} datasets, respectively. 

\subsubsection{Comparison Methods}

Here, we compare our propose approach MFGAN against a number of competitive baselines. 
% In this work, we propose a novel multi-factor enhanced GAN for sequential recommendation named MFGAN. By removing the external context information from MFGAN, we also implement a variant named SFGAN, which follows all the details of MFGAN,  where multiple discriminators degenerate into a single discriminator that only model transition pattern of origin item identifier.
Our baselines include related methods on general and sequential recommendation with or without context information:

$\bullet$ \textbf{PopRec}: This is a method that sorts items by their popularity to assign each item a rank, tending to recommend highly popular items to users.

 $\bullet$ \textbf{BPR}~\cite{Rendle-09-bpr}: This is a classic personalized ranking algorithm that optimizes the pairwise ranking loss function of latent factor model with implicit feedback.

$\bullet$ \textbf{FM}~\cite{FM2012}: It uses a generic matrix factorization to learn the coefficients of combined features, considering the interactions between different features.

$\bullet$ \textbf{IRGAN}~\cite{IRGAN}: This method combines generative and discriminative information retrieval via adversarial training, in which a simple matrix factorization is used for the discriminator.

$\bullet$ \textbf{FPMC}~\cite{RendleFS10}: It combines Matrix Factorization and Markov Chain, which can simultaneously capture sequential information and long-term user preference.

$\bullet$ \textbf{GRU}~\cite{GRU4Rec}: It is a GRU-based sequential recommender with session-parallel mini-batch training, which employs ranking-based loss functions. We implement an enhanced version by replacing one-hot vectors with pre-trained BPR vectors.

$\bullet$ \textbf{GRU$_F$}~\cite{GRU-f}: It proposes to incorporate additional feature vector as the input of GRU networks, which incorporates auxiliary features to improve sequential recommendation.

$\bullet$ \textbf{SASRec}~\cite{kang2018self}: It is a next-item sequential recommendation method based on the Transformer architecture, which adaptively considers interacted items for prediction. This method is the state-of-the-art baseline for sequential recommendation. 

$\bullet$ \textbf{MFGAN}: This is our approach introduced in Section~\ref{sec:method}.
%  \item \textbf{SFGAN}: This is our approach introduced in Section~\ref{sec:method} which only utilizes the single discriminator without context information.
% \noindent $\bullet$ \textbf{MFGAN}: This is our approach introduced in Section~\ref{sec:method}.

Besides GRU$_F$,  there are other baselines that utilize context information. However,  we have empirically found that the Transformer architecture is more superior than other sequence neural networks in sequential recommendation. Indeed, SASRec is significantly better than quite a few context-aware recommendation algorithms with other RNN architectures. 
%we have empirically found that SASRec  is particularly competitive, which can even beat quite a few context-aware sequential recommendation algorithms. 
%We speculate that it is due to the superiority of the Transformer architecture.
Therefore, our focus is how our approach improves over SASRec, and we omit other context-aware  baselines. Another note is that in comparison our MFGAN approach only utilizes the generator to recommend items, \ie context information or discriminators will not be used at the test stage. 

\subsection{Results and Analysis}
%\textsc{MovieLens-1M}, \textsc{Yahoo!} and \textsc{Steam} datasets, respectively. 


The results of different methods for sequential recommendation are presented in Table~\ref{tab:results-all}. It can be observed that:

(1) Among non-sequential recommendation baselines, we can find that BPR outperforms other methods, and  non-sequential recommendation methods overall perform worse than sequential recommendation methods.
Specially, factorization machine~(FM) does not work very well in this task, since it still adopts the regression loss and cannot effectively capture the preference order over two items by a user. Besides, popularity seems to be a robust baseline that gives substantial performance on our datasets. A major reason is that there may exist the ``\emph{rich-gets-richer}'' phenomenon in product adoption, and using $k$-core preprocessing on our datasets further enhances this trend.  


(2) Among sequential recommendation baselines, the Markov Chain-based method performs better on sparse dataset (\ie the game dataset) than dense datasets (\ie the other two datasets).
As for two neural methods, GRU adopts the RNN-based architecture, serving as a standard comparison method for sequential recommendation. With available context information, GRU$_F$ further improves over the GRU method, indicating context information is useful in our task.
Furthermore, SASRec utilizes the powerful Transformer architecture to develop the sequential recommender, achieving the best performance among all the baselines. 
In natural language processing, self-attention architecture has shown its superiority in various tasks~\cite{bert, transformer}. Such an architecture is particularly useful when dealing with sequence data, which also works well in sequential recommendation. 
%and SASRec utilizes the self-attention network, which gives better performance than GRU. Presumably self-attentive method can adaptively attend items within different ranges on different datasets and SASRec also gives the best performance among all the baselines. 

(3) Finally, we compare our proposed model MFGAN with  the baseline methods. It is clear to see that MFGAN is consistently better than these baselines by a large margin. Our base architecture is a pre-trained self-attentive generator. Different from the above models, we adopt the multi-adversarial architecture to guide the learning of the generator with various kinds of factor information. Note that 
our generator has not directly used any context information, and it is guided by the signals from the  discriminators. 
%Hence, we can form a fairness comparison our approach only utilizes the context information in the discriminators, and the generator is similar to the SASRec.
 Such a comparison indicates the multi-adversarial training approach is effective to improve the performance of self-attention architecture for sequential recommendation. 


\begin{figure*}[ht]
	\centering
	\subfigure[\textsc{Movielens-1m} movie dataset.]{\label{fig-ablation-movie}
		\centering
		\includegraphics[width=0.25\textwidth]{fig/ablation-movielens.pdf}
	}
	\subfigure[\textsc{Yahoo!} music dataset.]{\label{fig-ablation-music}
		\centering
		\includegraphics[width=0.25\textwidth]{fig/ablation-music.pdf}
	}
	\subfigure[\textsc{Steam} game dataset.]{\label{fig-ablation-game}
		\centering
		\includegraphics[width=0.25\textwidth]{fig/ablation-game.pdf}
	}
	\caption{Effect of different kinds of factor information in our framework for sequential recommendation. We report the results using the NDCG@10 metric. ``$\neg$'' indicates that we remove the corresponding factor information, while the rest factor information is kept. }
	\label{fig-ablation}
\end{figure*}

\ignore{For fairness comparison with SASRec, we only use the 
 utilize the context information of items, which is an elaborative way to make use of the context data. We only utilize the context data in the discriminators, while the implicit space that the generator models is isolated from context data. The generator is improved according to the feedback of the discriminator, which can be considered as indirect signal from context data.}

\eat{
\begin{table}[htbp]
  \centering
  \caption{Ablation analysis on the Movielens-1m dataset. There are four discriminators used in this dataset corresponding to four factors. We gradually increase the number of corresponding discriminator in order of identifier, semantics, category and popularity.}
  \label{tab:movie-ablation}%
    \begin{tabular}{l p{1.3cm}<{\centering} p{1.3cm}<{\centering} p{1.3cm}<{\centering}}
		\toprule
		Architecture            & NDCG@10 & HR@10 & MRR \\
		\midrule
		Default                 & \textbf{0.6185} & \textbf{0.8318} & \textbf{0.5587} \\
		\hline
		Single Discriminator    & 0.6032 & 0.8212 & 0.5413 \\
		Double Discriminators   & 0.6064 & 0.8232 & 0.5459 \\
		Remove ID               & 0.6156 & 0.8312 & 0.5506 \\
		Remove KG               & 0.6076 & 0.8245 & 0.5471 \\
		Remove Cat              & 0.6099 & 0.8247 & 0.5499 \\
		Remove Pop              & 0.6132 & 0.8298 & 0.5523 \\
		\hline
		Single-directional      & 0.6158 & 0.8299 & 0.5558 \\
		Min Reward              & 0.6117 & 0.8238 & 0.5525 \\
		\bottomrule
    \end{tabular}%
\end{table}%

\begin{table}[htbp]
  \centering
  \caption{Ablation analysis on the music dataset. There are five discriminators used in this dataset corresponding to five factors. We gradually increase the number of corresponding discriminator in order of identifier, artist, category, popularity and album.}
  \label{tab:music-ablation}%
    \begin{tabular}{l p{1.3cm}<{\centering} p{1.3cm}<{\centering} p{1.3cm}<{\centering}}
		\toprule
		Architecture            & NDCG@10 & HR@10 & MRR \\
		\midrule
		Default                 & \textbf{0.8556} & \textbf{0.9417} & \textbf{0.8286} \\
		\hline
		Single Discriminator    & 0.8478 & 0.9353 & 0.8207 \\
		Double Discriminators   & 0.8501 & 0.9395 & 0.8224 \\
		Triple Discriminators   & 0.8515 & 0.9407 & 0.8238 \\
		Remove ID               & 0.8536 & 0.9393 & 0.8271 \\
		Remove Artist           & 0.8522 & 0.9399 & 0.8251 \\
		Remove Cat              & 0.8541 & 0.9403 & 0.8274 \\
		Remove Pop              & 0.8532 & 0.9370 & 0.8274 \\
		Remove Album            & 0.8526 & 0.9380 & 0.8262 \\
		\hline
		Single-directional      & 0.8508 & 0.9396 & 0.8231 \\
		Min Reward              & 0.8493 & 0.9431 & 0.8201 \\
		\bottomrule
    \end{tabular}%
\end{table}%

\begin{table}[htbp]
  \centering
  \caption{Ablation analysis on the game dataset. There are five discriminators used in this dataset corresponding to five factors. We gradually increase the number of corresponding discriminator in order of identifier, development, category, popularity and price.}
  \label{tab:game-ablation}%
    \begin{tabular}{l p{1.3cm}<{\centering} p{1.3cm}<{\centering} p{1.3cm}<{\centering}}
		\toprule
		Architecture            & NDCG@10 & HR@10 & MRR \\
		\midrule
		Default                 & 0.6035 & \textbf{0.8488} & 0.5346 \\
		\hline
		Single Discriminator    & 0.5990 & 0.8426 & 0.5308 \\
		Double Discriminators   & 0.6008 & 0.8430 & 0.5321 \\
		Triple Discriminators   & 0.6009 & 0.8402 & 0.5336 \\
		Remove ID               & 0.6013 & 0.8450 & 0.5316 \\
		Remove Dev              & \textbf{0.6043} & 0.8467 & \textbf{0.5352} \\
		Remove Cat              & 0.6010 & 0.8456 & 0.5315 \\
		Remove Pop              & 0.6003 & 0.8457 & 0.5305 \\
		Remove Price            & 0.6009 & 0.8437 & 0.5319 \\
		\hline
		Single-directional      & 0.6006 & 0.8426 & 0.5321 \\
		Min Reward              & 0.6012 & 0.8434 & 0.5327 \\
		\bottomrule
    \end{tabular}%
\end{table}%
}




\subsection{Detailed Analysis on Our Approach}

In this section, we further conduct a series of detailed experiments to analyze the effectiveness of our approach.  

\subsubsection{Effect of Different Factors}
% \paratitle{Effect of Different Factors.}
In this part, we study the effect of different kinds of factor information in our approach. 
We first prepare the complete MFGAN model, and then remove one kind of factor information at each time. 
In this way, we can study how each individual factor contributes to the final performance for sequential recommendation. 
Figure~\ref{fig-ablation} presents the NDCG@10 results of factor removal experiments for MFGAN. 
As we can see, all the factors seem to be useful to improve the performance of our MFGAN, except the factor \emph{developer} on the \textsc{Steam} game dataset. The most useful factors are \emph{knowledge graph}, \emph{artist} and \emph{popularity} for the three datasets, respectively. %Such an observation is indeed consistent with our intuition. 
Interestingly,  item ID is not always  the most useful feature for discriminators, indicating the importance of other kinds of factor information.

\subsubsection{Comparisons of Model Variants}
% \paratitle{Comparisons of Model Variants.}
In our model, we propose several techniques to improve the performance of our approach. Here, we construct  comparison experiments to examine the effect of these techniques:
 (1) \underline{\emph{Uni-directional}} using a uni-directional self-attention architecture in discriminators; 
 %(2) \underline{\emph{Max-reward}} selecting the maximum reward from all the discriminators (Eq.~\ref{eq:action-value}); (3) \underline{\emph{Min-reward}} selecting the minimum reward from all the discriminators (Eq.~\ref{eq:action-value}); 
 (2) \underline{\emph{SDSF}} using  a single discriminator considering  item ID as the only factor; (3) \underline{\emph{SDAF}} using a single discriminator incorporating all factor embeddings using simple vector concatenation.
The first variant is used to illustrate the effect of the bi-directional architecture, %the next two variants are used to illustrate the effect of the reward aggregation method (recall that we adopt an average method to aggregate the reward signals), 
and the last two variants are used to illustrate the effect of using multiple discriminators. 

\begin{table}[htbp]
  \centering
  \caption{Variant comparisons of our MFGAN framework on \textsc{Movielens-1m} dataset.}
  \label{tab:ablation}%
    \begin{tabular}{l p{1.3cm}<{\centering} p{1.3cm}<{\centering} p{1.3cm}<{\centering}}
  \toprule
  Architecture            & NDCG@10 & HR@10 & MRR \\
  \midrule
  MFGAN                 & \textbf{0.6185} & \textbf{0.8318} & \textbf{0.5587} \\
  \hline
  SASRec                & 0.5849 & 0.8132 & 0.5214 \\
  Uni-Directional       & 0.6158 & 0.8299 & 0.5558 \\
 % Max-Reward            & 0.6122 & 0.8253 & 0.5527 \\
  %Min-Reward            & 0.6117 & 0.8238 & 0.5525 \\
  SDSF                  & 0.6032 & 0.8212 & 0.5413 \\
  SDAF                  & 0.6039 & 0.8221 & 0.5455 \\
  \bottomrule
    \end{tabular}%
\end{table}%

\begin{figure}[!tb]
	\small
	\centering 
	\includegraphics[width=0.37\textwidth]{fig/loss.pdf}
	\caption{Convergence of loss with different numbers of discriminators in \textsc{Movielens-1m} dataset.} %	\vspace{-0.3cm} 
	\label{fig-loss} 
\end{figure}

Table~\ref{tab:ablation} presents the comparisons of these variants against our complete approach and SASRec. We can see that all the variants are worse than the complete approach. It indicates that  the bi-directional architecture and  multi-discriminator adversarial training are effective to improve the performance.
However, the improvement with bi-directional architecture seems to be small in numerical values.
A possible reason is that the uni-directional Transformer architecture  is ready very competitive. 
While,   the idea that utilizes the bi-directional architecture in discriminators has important implications. As future work, it will be interesting  to design other architectures for generator and discriminator, respectively. %We believe that 
%, since the base architecture has already achieved a very competitive performance. Another possible reason is that these techniques are directly used by the discriminators, which indirectly affect the performance of the generator. 
%Although the yielded improvement is not significant,  the actual model capacity might have been enhanced substantially. %While, we argue these techniques are importan to cosnider 


\begin{figure*}[ht]
	\centering
	\subfigure[A case from \textsc{Movielens-1m} movie dataset.]{\label{fig-case-movie}
		\centering
		\includegraphics[width=0.49\textwidth]{fig/case_movie.pdf}
	}
	\subfigure[A case from \textsc{Yahoo!} music dataset.]{\label{fig-case-music}
		\centering
		\includegraphics[width=0.48\textwidth]{fig/case_music.pdf}
	}
	\caption{Two qualitative cases with our approach. In each figure, the upper part is the interaction sequence, and the lower part corresponds to the lines of reward signal scores from some factors. 
	The height of the histogram represents the reward score within the interval $(0,1)$. We use the red color to highlight the highest bar (\ie the dominant factor) at each time step. For the two cases, we mainly focus on the \emph{category} and \emph{artist} factor, respectively. }
	\label{fig-case}
\end{figure*}

Note that the \emph{SDSF} variant can be considered as an enhanced implementation of SeqGAN~\cite{Yu2017SeqGAN}, where the generator and the discriminator have been  improved using the Transformer architecture. SeqGAN is originally proposed for general sequence generation, while it is easy to adapt to our task. 

Besides the performance improvement, as discussed in Section~\ref{sec:method}, using multiple discriminators is likely to stabilize the training of adversarial learning approaches.  
For this purpose, we further compare the convergence of our objective function with a varying number of discriminators during training process.
As we can see in Fig.~\ref{fig-loss}, using more discriminators is faster to achieve a relatively stable loss. The red and green lines (corresponding to use three or four discriminators) become stable after about 2000 epochs, while the other lines are not stable even after 4000 epochs. Another interesting observation is that using more discriminators seems to yield a larger loss. We speculate that it has the similar effect of regularization, which prevents the model parameters from overfitting on training data. 
%In addition, we explore the convergence of the loss functions with different number of discriminators, shown in Fig.~\ref{fig-loss}. The result shows that with gradual increasing of the discriminator number, the convergence rate of loss gradually slows down. This illustrates that increasing the number of discriminators is a constraint on the convergence of loss.

\ignore{In order to better explore the impact of the number of discriminators on the experimental performance, we implement the experiment to examine how the performance changes after removing each factor.
With experimental results in Fig.~\ref{fig-ablation} corresponding to three datasets, we can find that full number discriminators architecture generally gets the best performance, after removing different discriminator corresponding to a factor causes different degrees of model performance degradation, this can be explained as different factors playing different roles in the task, which demonstrated the improvement of model effectiveness by multi-adversarial architecture.}


%\subsubsection{Reward: Soft vs Min}


\ignore{

In our model, we adopt multi-adversarial frameworks with discriminators corresponding to different factors and use softmax operator when integrating the multiple rewards and then return to the generator. We introduce a variant version, using min reward among all the rewards, denote that generator trains against the most strict discriminator which provides a harsher critic to the generator.
Fig.~\ref{fig-ablation} shows the performance comparing the softmax and the min operator, we can see that using min reward, the performance is worse than softmax reward and during the training process, the convergence is also unstable. The result demonstrates that adopting min reward is too harsh a critic, and it can impede the generator's learning. 
% Using a softmax also has the well-known advantage of being differentiable (as opposed to subdifferentiable for min). To increase the odds of providing constructive feedback to the generator, we set $\lambda$ to zero to apply the mean option in eq.~\ref{eq:action-value}.



\subsubsection{Bi-directional vs Uni-directional}
In this part we explored the impact of the bi-directional self-attention mechanism on model performance in the discriminators. Uni-directional model masks the item behind timestamp $t$, only considers the item before $t$, we modify the self-attention in discriminators by forbidding all links between $\mathbf{Q}_i$ and $\mathbf{K}_j$ ($j > i$). The results are showed in Fig.~\ref{fig-ablation}. We account that the unmasked model can consider more future information. 
Perhaps because the discriminative task is not very difficult, applying the uni-directional discriminator has not made a particularly large impact on the results, just impairs a little bit of performance, but it still proves the effectiveness of the bi-directional architecture compared to the uni-directional architecture.
}



\subsection{Qualitative Analysis on the Recommendation Interpretability}
Previous experiments have verified that our model is able to generate high-quality sequential recommendations. Another major benefit of our work is that our recommendations are highly interpretable due to the decoupled factors in the multi-adversarial framework. 
Here, we present two illustrative examples in Fig.~\ref{fig-case}, showing how our approach improves the recommendation interpretability with decoupled factors.

%As a case study, we present examples from the datasets in Fig.~\ref{fig-case}, which shows two interaction sequences of several records. Each record consists of two parts: the top part corresponds to the information of the item and the bottom part corresponds to the rewards obtained from different discriminators, which can indicate which factor is dominant in the user's choice at current timestamp.
The first case (Fig.~\ref{fig-case-movie}) presents an interaction sequence of a sample user from \textsc{Movielens-1m} dataset. As we can see, the first two movies ``\emph{Star War: episode VI}'' and ``\emph{E.T. the Extra-Terrestrial}'' have received  higher reward signals from \emph{popularity}, which is the prominent factor at the beginning stage. Interestingly, seen from the \emph{category} line,  the $3$-rd, $6$-th and $7$-th movies are mainly driven by the category factor. Given the the last two movies ``\emph{Star War: episode IV}'' and ``\emph{Star War: episode V}'', the user, influenced by early popularity, seems to be a Star Wars fan or an action movie fan.%, which is  influenced by early trend of the first movie.

\ignore{Fig.~\ref{fig-case-movie} presents an interaction sequence of a sample user from movielens-1m. Firstly, the user started with the movie \emph{Star War: episode VI}, which is an action movie. Then, he watched a Sci-Fi movie. The popularity of the first two movies is relatively high, so the model believes that the selection of these two movies is dominated by popularity.
For the third movie, he switched to \emph{Jurassic Park}, which is also an action movie, at this timestamp, the model captures through the feedback of the multiple discriminators that the user chose \emph{Jurassic Park} because of the category of the movie. 
Subsequently, the fourth and fifth movies are drama and thriller. For the last two movies, the user selected \emph{Star War: episode IV} and \emph{Star War: episode V} in turn, our model finds out exactly that he most likely chose these two movies because of the category, and the interesting point is that we can find this user is likely to be a Star Wars fan or an action movie fan.}

The second case (Fig.~\ref{fig-case-music}) presents an interaction sequence of a sample user from \textsc{Yahoo!} music dataset. 
Similarly, we can check the effect of multiple factors at different time steps. 
Here, we mainly analyze the \emph{artist} factor,  focusing on the 4-th, 6-th and 7-th songs.
Along the interaction sequence, this user switches among different artists. Our model is able to capture such listening patterns: 
when the user listens to a song of a previous artist (\ie previously appearing in the interaction sequence) occurs, the corresponding \emph{artist} factor becomes dominant in our model. 

As a comparison, existing methods mainly focus on integrating various kinds of context information into  unified representations. The two examples have shown the advantage of decoupling various factors for sequential recommendation. %It is flexible to incorporate other kinds of factors and monitor the effect of some specific factors. 


\ignore{The user started with three songs by different artists, note that the first artist is one of the user's frequent artists, our model thinks that the user listened to the song because of the first artist. The second artist and the third artist are not the artists he often listens to. This user is accustomed to listening to a few artists and rarely to others, when he listens to the songs by a frequent artist, the model generally thinks that the artist factor is dominant when he listens to the current song. When he does not listen to a fixed artist's song, it will considered to be dominated by identifier co-occurrence of the song.
Once the user listens to a song by an infrequent artist, the model will capture that artist is the dominant factor sensitively.

Through the illustrations above, we demonstrate that by decoupling the interactive information through multiple discriminators, we can know which factor is dominated of the user when selecting the item at each timestamp, and we can also know which factors are considered more when recommending items to a user.
}

% \subsubsection{Combining multiple discriminators as a ``generator''}
% \yaliang{Experimentally confirm the motivation of decoupling multiple factors from ID information}

% \subsection{Training Strategies}


==> Sequential Recommendation with Self-Attentive Multi-Adversarial Network/subfile2/5_related.tex <==
\section{Related Work}
\label{sec:related}
 In this section, we review studies closely related to our work in two aspects.

\eat{
In this section, we review several lines of related works, including sequential models, and generative adversarial network.}

\eat{
\paratitle{General Recommendation.} 
Early recommendation systems were designed to model users and items with implicit feedback~\cite{KorenBV09} or explicit feedback~\cite{Rendle-09-bpr}. A classical method is collaborative filtering (CF), using the interests of a group with similar interests to recommend information that users are interested in~\cite{HerlockerKBR99, SarwarKKR01}. Moreover, FM~\cite{FM2012} can imitate most decomposition models through feature engineering.
Due to the success in some areas, deep learning techniques have been introduced to recommendation system. A typical work is NCF~\cite{NCF17}, which uses DNN to simulate noise implicit feedback signals. AutoRec~\cite{SedhainMSX15} uses the autoencoder model to predict missing ratings in the user-item matrix.
}

\paratitle{Sequential Recommendation.}
% The goal of sequential recommendation is to predict the next item(s) that a user will interact with based on historical behaviors.
Early works on sequential recommendation are mainly based on Markov Chain (MC) assumption.
For instance, Rendle et al.~\cite{RendleFS10} fuse the matrix factorization and first-order Markov Chain for modeling global user preference and short-term interests, respectively.
%Since user behaviors are tightly related to the last one interaction, first-order Markov Chain has achieved remarkable success, especially on sparse datasets.
%By attending information from the previous interactions layer by layer, Caser is capable of compressing the longer-term item transitions.
Another line to model user behaviors is resorting to the recurrent neural network, which has achieved  great success on sequential modeling in a variety of applications.
Hidasi et al.~\cite{GRU4Rec} firstly introduce Gated Recurrent Units (GRU) to the session-based recommendation.
A surge of following variants modify it by introducing pair-wise loss function~\cite{GRU-f}, attention mechanism~\cite{LiRCRLM17}, memory network~\cite{chen2018sequential}, hierarchical structure~\cite{QuadranaKHC17}, etc.
Other architectures or networks have also been used~\cite{lv2019sdm,ma2019hierarchical}, achieving good performance.
Moreover, context information is often used to improve the recommendation performance and interpretability~\cite{GRU-f, wang2017context, Huang-2018-SIGIR, HuangWSDM19}.
Recently, self-attention network has achieved significant improvement in a bunch of NLP tasks~\cite{transformer, bert} and inspired a new direction on applying the self-attention mechanism to sequential recommendation problem~\cite{kang2018self}.
% SASRec~\cite{kang2018self} proposes to utilize the self-attentive architecture to capture  dependencies of user's historical behaviors.
%Despite of remarkable success of these proposed sequential recommendation models, black-box model structures conversely hinder the understanding of user behaviors in trajectories.
% Sun et al.~\cite{bert4rec} extend it with the introduction of Cloze task~\cite{Cloze} and bidirectional supervision.

\ignore{
\paratitle{Explainable Recommendation.} 
Explainable recommendation refers to personalized recommendation algorithms that address the problem of why~\cite{DBLP:journals/corr/abs-1804-11192}. The term of explainable recommendation was formally introduced in recent years~\cite{ZhangL0ZLM14}, and a large number of explainable recommendation approaches have been proposed and applied in real-world systems, simply classified as matrix factorization explainable recommendation~\cite{ZhangL0ZLM14}, graph-based explainable recommendation~\cite{HeckelVPD17}, knowledge-based explainable recommendation~\cite{Huang-2018-SIGIR, WangWX00C19}, rule mining explainable recommendation~\cite{BalogRA19}, etc.
}

\paratitle{Generative Adversarial Network.} 
Generative Adversarial Network (GAN)~\cite{GAN-2014-NIPS} was originally proposed to mimic the generation process of given data samples.
Typically, GAN consists of two components: the generative model learns to map from a latent space to a data distribution of interest, while the discriminative model distinguishes candidates produced by the generator from the true data distribution.
A surge of follow-up works either improve the GAN framework by introducing more advanced training strategies, like f-divergence~\cite{f-gan}, Wasserstein distance~\cite{WuHTAG18}, MMD constraints~\cite{li2017mmd} or explore diverse applications under GAN framework~\cite{SRGAN,Yu2017SeqGAN,ZhangGFCHSC17}.
%In the field of computer vision and natural language processing, it has yielded a variety of promising applications~\cite{singan,cartoongan,SRGAN,Yu2017SeqGAN,KusnerH16,ZhangGFCHSC17} while it has not gained much attention in recommender system. 
In recommender systems, the idea of GAN has already been explored to some extent. 
IRGAN~\cite{IRGAN} is firstly proposed to unify the generative model and discriminative model in the field of information retrieval.
Chae et al.~\cite{CFGAN} follow this line and further improve the training scheme by sampling a real-valued vector instead of a single item index.
Moreover, personalized determinantal point process is utilized to improve recommendation diversity via adversarial training~\cite{WuLMZZG19}.
%Although they have achieved promising improvements on recommendation performance or relevance, they are generally tailored for traditional matrix factorization techniques and thus ignore the valuable temporal information of user behaviors.

Our work is related to the above studies, while has a different focus. 
We are the first to apply adversarial training to sequential recommender systems. 
By designing a multi-adversarial network, our model is able to explicitly characterize the effect of each individual factor on sequential recommendation over time, which improves the recommendation interpretability.  

\eat{
PD-GAN~\cite{WuLMZZG19} furtissues the problem of the diversity problem while largely preserve or even boost relevance by adversarial training.
With the recent successes of Generative Adversarial Network~\cite{GAN-2014-NIPS, gan-survey}, it has been one of the most breakthrough technique on genera in recent years

With the recent successes of GANs~\cite{GAN-2014-NIPS, gan-survey}, the GAN framework has been one of the most breakthrough learning technique in recent years, which The total process while adversarial training is a min-max game between the generator and the discriminator. A set of constraints are proposed in previous works~\cite{RadfordMC15, HuangLPHB17, RadfordMC15, WuHTAG18, GeXCBW18} to improve the training process of GANs, and GAN-based methods are also applied in NLP tasks~\cite{Yu2017SeqGAN, KusnerH16, ZhangGFCHSC17, GuoLCZYW18}. 
Recently, there are quite a few studies that utilize GAN in recommendation system, such as IRGAN~\cite{IRGAN}, which unify the generative retrieval model and the discriminative retrieval model through GAN framework, including recommendation task, and CFGAN~\cite{CFGAN} improve collaborative filtering with adversarial training. Both two methods base on matrix factorisation and do not consider the temporal information. Besides, PD-GAN~\cite{WuLMZZG19} improves recommendation diversity while largely preserve or even boost relevance by adversarial training.
To our knowledge, there is no work currently applies GAN in sequential recommendation.


Different from the above approaches in that they only model the item-level sequences or they not fit enough for our task, we first introduce adversarial training into the sequential recommendation task, use bidirectional discriminator to enhance the supervision during the generation process, and we propose a multi-adversarial architecture with multiple factors, further strengthen the supervision from different perspectives to improve the performance of sequential recommendation. Besides, by decoupling different factor information from the discrimination side, our model can strip out what factor the user is affected by when selecting the item, making the model interpretable.
}






==> Sequential Recommendation with Self-Attentive Multi-Adversarial Network/subfile2/6_conclusion.tex <==
\section{Conclusions}
\label{sec:conclusions}

In this paper, we have proposed a Multi-Factor Generative Adversarial Network (MFGAN) for sequential recommendation. In our framework, the generator taking user behavior sequences as input is used to 
generate possible next items, and multiple factor-specific discriminators are used to evaluate the generated sub-sequence from the perspectives of different factors. We have constructed extensive experiments
on three real-world datasets. Experimental results have shown that our approach outperforms several competitive baselines. Especially, we have found that using multiple discriminators is useful to stabilize the training of adversarial learning, and also enhance the interpretability of recommendation algorithms. 


Currently, we consider a simple setting where multiple discriminators are separately designed. As future work, we will investigate how to design a more principled way to share discrimination information across different discriminators. We will also consider incorporating explicit user preference in the discriminators.  
